A Stochastic Nonlinear Model Predictive Control with an Uncertainty Propagation Horizon for Autonomous Vehicle Motion Control

Employing Stochastic Nonlinear Model Predictive Control (SNMPC) for real-time applications is challenging due to the complex task of propagating uncertainties through nonlinear systems. This difficulty becomes more pronounced in high-dimensional systems with extended prediction horizons, such as autonomous vehicles. To enhance closed-loop performance in and feasibility in SNMPCs, we introduce the concept of the Uncertainty Propagation Horizon (UPH). The UPH limits the time for uncertainty propagation through system dynamics, preventing trajectory divergence, optimizing feedback loop advantages, and reducing computational overhead. Our SNMPC approach utilizes Polynomial Chaos Expansion (PCE) to propagate uncertainties and incorporates nonlinear hard constraints on state expectations and nonlinear probabilistic constraints. We transform the probabilistic constraints into deterministic constraints by estimating the nonlinear constraints' expectation and variance. We then showcase our algorithm's effectiveness in real-time control of a high-dimensional, highly nonlinear system-the trajectory following of an autonomous passenger vehicle, modeled with a dynamic nonlinear single-track model. Experimental results demonstrate our approach's robust capability to follow an optimal racetrack trajectory at speeds of up to 37.5m/s while dealing with state estimation disturbances, achieving a minimum solving frequency of 97Hz. Additionally, our experiments illustrate that limiting the UPH renders previously infeasible SNMPC problems feasible, even when incorrect uncertainty assumptions or strong disturbances are present.

==> sections/real_results.tex <==
% \subsection{EDGAR sensor setup}
% % TODO:  cite edgar  paper
% % TODO: EDGAR small Photo
% \subsection{experiment setup}
% Double Lane Change according to ISO 3888-1:2011

==> sections/related_work.tex <==
% keep it short only about SNMPC:
% start with 2012 (Fagiano) \cite{fagiano2012nonlinear}, 2014 (Mesbah) \cite{mesbah2014stochastic}, 2014 (Streif) 
% go on the difference and the evolotution between the different papers then introduce the evolution/upgrade we do in this paper. 


% - Dealing with disturbances
% - Dealing with disturbances in NMPC
% - Robust NMPC
% - Stochastic Linear MPC
% - Stochastic NMPC
% - Motion control application (disturbances + NMPC / disturbances + MPC)
% \cite{falcone2007linear} 

% The rest of the paper is structured as follows. In Sec.\ref{sec:nominal_nmpc}, ... 

Stochastic uncertainties are nonnegligible in complex dynamic system and can cause unpredicted and undesired system output if a nominal NMPC is used, hence lead a bad closed-loop performance. To handle these uncertainties, two variant of NMPC, namely Robust NMPC and stochatic NMPC can be applied.

Robust NMPC assumes bounded uncertainties and enables analyzing the stability and performance of the system against worst-case perturbations. This has led to a number of applications, where providing guarantees on robust stability and performance is the main objective [1], [2]. However, the worst-case perturbations may have a extremely small probability of occurrence in real practice [3], so control design based on worst-case uncertainties can be too conservative and, therefore, may lead to infeasible control problems. In addition, it is seldom practical to specify precisely the uncertainty bounds.

In contrast, SNMPC with chance constraints adopts a distinctive strategy to solve MPC problems under uncertainties. It ultilizes probabilistic descriptions of uncertainties and constraint violations, allowing for acceptable levels of risk during system operation. Chance constraints offers the possibility to trade off between closed-loop performance and constraints violation, which mitigate the inherent conservativeness in robust NMPC.

Unlike linear SMPC, SNMPC has been much less developed due to the difficulty in efficient UP through nonlinear system. SNMPC can be broadly categotized in terms of the underlying UP method. The use of Markov-chain Monte Carlo \cite{maciejowski2007nmpc} techniques was initially proposed that didn't rely on convexity assumptions and guaranteed convergence to near-optimal solutions under certain conditions related to the convergence of a homogeneous Markov chain. However, their effectiveness when implemented in a receding-horizon manner remained unproven. Sequential Monte Carlo was adopted in \cite{kantas2009sequential} to further improve effectiveness.

To deal with the difficulties of efficient UP, Gaussian-mixture approximation method \cite{weissel2009stochastic} was used to describe the transition probability distributions of states. This approach allowed for a flexible framework for constructing the probability distributions of stochastic variables, enabling a more comprehensive representation of uncertainty.

The gPC approach \cite{fagiano2012nonlinear} \cite{mesbah2014stochastic} was afterwards proposed to address time-invariant stochastic uncertainties in both system parameters and initial conditions. The gPC framework replaces the conventional implicit mappings between uncertain variables/parameters and states, providing an efficient method for predicting the time evolution of the moments of probability distributions of stochastic states.

All works using gPC framework aims to control a system in a relative stable environment with a fixed control objective under uncertainty. In this work, we further extend this framework to a motion control application with a novel UPH concept, which helps stabilizing SNMPC during UP. This application aims to make a vehicle with highly nonlinear dynamics track a time-varying reference trajectory, which means both external environent and control objective vary frequently over time.

The rest of paper is structured as follows. In \ref{sec:nominal_nmpc}, the nominal NMPC problem will be formulated. Afterwards, \ref{sec:stochastic_nmpc} introduces the implementations and novelty of this paper. In \ref{sec:traj_following} the formulation of trajectory following application will be presented and the simulation results will be discussed in \ref{sec:sim_results}. At last, we will conclude the results and give a outlook for further research.
